A Statistical Framework for Data-dependent Retrieval-Augmented Models

Modern ML systems increasingly augment input instances with additional relevant information to enhance final prediction. Despite growing interest in such retrieval-augmented models, their fundamental properties and training are not well understood. We propose a statistical framework to study such models with two components: 1) a {\em retriever} to identify the relevant information out of a large corpus via a data-dependent metric; and 2) a {\em predictor} that consumes the input instances along with the retrieved information to make the final predictions. We present a principled method for end-to-end training of both components and draw connections with various training approaches in the literature. Furthermore, we establish excess risk bounds for retrieval-augmented models while delineating the contributions of both retriever and predictor towards the model performance. We validate the utility of our proposed training methods along with the key takeaways from our statistical analysis on open domain question answering task where retrieval augmentation is important.

==> 070_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Despite the widespread empirical success of RAMs, a rigorous understanding of their basic properties such as their generalization behavior and expressive power are far from well understood. Similarly, even though numerous domain-specific procedures to train RAMs have been proposed in the literature, a unified training framework for these models that can leverage advancement in the broader field of ML has received limited attention.

